Revisit Systematic Generalization via Meaningful Learning

Humans can systematically generalize to novel compositions of existing concepts. Recent studies argue that neural networks appear inherently ineffective in such cognitive capacity, leading to a pessimistic view and a lack of attention to optimistic results. We revisit this controversial topic from the perspective of meaningful learning, an exceptional capability of humans to learn novel concepts by connecting them with known ones. We reassess the compositional skills of sequence-to-sequence models conditioned on the semantic links between new and old concepts. Our observations suggest that models can successfully one-shot generalize to novel concepts and compositions through semantic linking, either inductively or deductively. We demonstrate that prior knowledge plays a key role as well. In addition to synthetic tests, we further conduct proof-of-concept experiments in machine translation and semantic parsing, showing the benefits of meaningful learning in applications. We hope our positive findings will encourage excavating modern neural networks' potential in systematic generalization through more advanced learning schemes.

==> [BlackboxNLP 2022] Revisit Systematic Generalization via Meaningful Learning/1.abstract.tex <==
\begin{abstract}
\vspace{-1mm}
Humans can systematically generalize to novel compositions of existing concepts. Recent studies argue that neural networks appear inherently ineffective in such cognitive capacity, leading to a pessimistic view and a lack of attention to optimistic results. We revisit this controversial topic from the perspective of meaningful learning, an exceptional capability of humans to learn novel concepts by connecting them with known ones. We reassess the compositional skills of sequence-to-sequence models conditioned on the semantic links between new and old concepts. Our observations suggest that models can successfully one-shot generalize to novel concepts and compositions through semantic linking, either inductively or deductively. We demonstrate that prior knowledge plays a key role as well. In addition to synthetic tests, we further conduct proof-of-concept experiments in machine translation and semantic parsing, showing the benefits of meaningful learning in applications. We hope our positive findings will encourage excavating modern neural networks' potential in systematic generalization through more advanced learning schemes.
\vspace{-2mm}
\end{abstract}

==> [BlackboxNLP 2022] Revisit Systematic Generalization via Meaningful Learning/2.introduction.tex <==
\vspace{-1mm}
\section{Introduction}
\vspace{-1mm}

\begin{figure}[t]
    \begin{center}
        \includegraphics[width=\linewidth]{figures/blk_nlp-scan_1.drawio.pdf}
        \vspace{-8mm}
    \end{center}
    \caption{An example of the one-shot compositional generalization from the old concept ``\textit{\textbf{walk left}}'' to the new one ``\textit{\textbf{turn left and walk}}'' in SCAN. The model is able to generalize from the command ``\textit{\textbf{walk left} and jump left}'' to ``\textit{\textbf{turn left and walk} and jump left}'' through the semantic relationship between the old and new concepts because they refer to the same action ``\textbf{LTURN WALK}''. Such semantic linking can be established by either an inductive sample or a deductive rule.}
    \label{figure:scan}
    \vspace{-5mm}
\end{figure}

% opening words
As a crucial characteristic of human cognition, systematic generalization reflects people's talents to learn infinite combinations of finite concepts \citep{chomsky1957syntactic,montague1970universal}. Whether connectionist networks can express language and thoughts systematically has been controversial for many years \citep{fodor1988connectionism,hadley1994systematicity,marcus1998rethinking,fodor2002compositionality,brakel2009strong,frank2009connectionist,marcus2018algebraic}. To date, the systematic compositionality in neural networks remains an appealing research topic. Evidence on multiple explicitly proposed language-based generalization challenges suggests that models lack such cognitive capacity \citep{bastings-etal-2018-jump,loula-etal-2018-rearranging,sinha-etal-2019-clutrr,keysers2020measuring,hupkes2020compositionality,kim-linzen-2020-cogs,li-etal-2021-compositional}. Tremendous efforts are made to tackle these challenges through architectural modifications \citep{li-etal-2019-compositional,Gordon2020Permutation,oren-etal-2020-improving,akyurek-andreas-2021-lexicon,chaabouni-etal-2021-transformers}, meta-learning \citep{NEURIPS2019_f4d0e2e7,conklin-etal-2021-meta}, grammar \citep{kim2021sequence,shaw-etal-2021-compositional}, neuro-symbolic models \citep{ChenLYSZ20,NEURIPS2020_83adc922,NEURIPS2020_7a685d9e}, data augmentation \citep{andreas-2020-good,rek2021learning,auersperger-pecina-2021-solving,jiang-bansal-2021-inducing,patel-etal-2022-revisiting}, and loss design \citep{yin-etal-2021-compositional}. Despite their astounding accomplishments, standard sequence-to-sequence (seq2seq) models \citep{sutskever2014sequence} appear to have relatively weak inductive biases, failing to capture underlying hierarchical structure.

\begin{figure*}[t]
    \begin{center}
        \includegraphics[width=\textwidth]{figures/blk_nlp-ml.drawio.pdf}
        \vspace{-8mm}
    \end{center}
    \caption{Adapted examples from Geography. In the left one, intuitively, knowing how the new concept (e.g., ``\textit{USA}'') relates to the other existing ones (e.g., ``\textit{US}'') can boost the learning and memory of this knowledge as a whole. In the right one, bidirectional arrows denote symmetric relations. ``\textit{Mississippi}'' and ``\textit{California}'' are two specific states, and thus both are hyponyms of ``\textit{state}''. In turn, ``\textit{state}'' is a hypernym of them. Due to a common hypernym, ``\textit{Mississippi}'' and ``\textit{California}'' become a co-hyponym for each other. \{``\textit{heavily populated}'', ``\textit{congested}'', ``\textit{populus}''\} is a group of synonyms as sharing similar semantics. Finally, ``\textit{U.S.}'', as a kind of abbreviation, is a lexical variant of ``\textit{United States}''.}
\label{figure:ml}
\vspace{-5mm}
\end{figure*}

In contrast, the successful one-shot generalization in the turn-left experiment on the \textbf{S}implified \textbf{C}omm\textbf{A}I \textbf{N}avigation (SCAN) task reveals the potential of seq2seq recurrent networks in controlled environments \citep{lake2017generalization}. Although models are only exposed to the primitive command before, they are able to understand most composed commands of ``\textit{turn left}''. One assumption is that models study new commands with a primitive from other action sequences containing the basic action it denotes. However, there is still a missing formal exploration to answer the question raised by \citet{lake2017generalization} on page 8 that ``\emph{what are, precisely, the generalization mechanisms that subtend the networks’ success in these experiments}''.

In this work, as a response to the call, we question whether neural networks are indeed deficient or just conventional learning protocols unable to exploit their full potential \citep{csordas2021devil,dankers-etal-2022-transformer}. We revisit the systematic generalization of seq2seq models from a \emph{meaningful learning} perspective \citep{ausubel1963psychology,okebukola1988cognitive,mayer2002rote}. Given the idea that humans are used to memorizing concepts in a relational manner, we hypothesize that the success of the turn-left experiment results from the semantic relationships between old concepts and new ones. For example, in Figure \ref{figure:scan}, a model can understand the meaning of ``\textit{\textbf{turn left and walk} and jump left}'' from ``\textit{\textbf{walk left} and jump left}'' via the semantic link between two concepts (in bold) since both denote to the same action ``LTURN WALK''.

To validate our hypothesis, we reproduce the one-shot compositional generalization by \emph{semantic linking} that exposes semantic relationships through either \emph{inductive learning} or \emph{deductive learning} \citep{hammerly1975deduction,shaffer1989comparison,thornbury1999teach}. On the one hand, by introducing new concepts sharing the same context, we hope the model can capture the underlying semantic connections inductively. On the other hand, by involving a rule-like concept dictionary without specific context information, we hope the model can utilize the general cross-lingual supervised signals as anchor points so as to launch the semantic linking deductively.

In experiments, we treat concepts in the initial data set as primitives and generate variant samples and rules accordingly. Next, we mix them up and construct a seq2seq task after a random split. We repeatedly train and evaluate models but slowly decrease the number of times they see each variant until one-shot learning. We observe there is hardly a performance drop in SCAN for three representative model structures. This evidences that, with semantic linking, even canonical neural networks can generalize systematically to new concepts and compositions. Such observation holds consistently across two more semantic parsing (SP) datasets. The followed sensitivity analysis shows that prior knowledge also takes essential parts. Lastly, as a proof-of-concept, we demonstrate how meaningful learning already benefits models in standard machine translation (MT) and SP. Overall, our contributions\footnote{Code and data are publicly available at \href{https://github.com/ShiningLab/Systematic-Generalization-via-Meaningful-Learning}{GitHub}.} are as follows:
\begin{itemize}[leftmargin=*,noitemsep,topsep=0pt]
    \item We revisit systematic generalization from a meaningful learning perspective by either inductive or deductive semantic linking.
    \item We find that modern seq2seq models can generalize to new concepts and compositions after semantic linking, which empirically answers the question by \citet{lake2017generalization}.
    \item We show in the sensitivity analysis that both semantic linking and prior knowledge play a key role, in line with meaningful learning theory.
    \item We extend to standard MT and SP and demonstrate how meaningful learning already benefits models in solving realistic problems.
\end{itemize}

==> [BlackboxNLP 2022] Revisit Systematic Generalization via Meaningful Learning/3.meaningful_learning.tex <==
% \vspace{-2mm}
\section{Meaningful Learning}
% \vspace{-2mm}

In educational psychology, meaningful learning refers to learning new concepts by relating them to old ones \citep{ausubel1963psychology,mayer2002rote}.
% On the contrary, rote learning stands for learning new concepts without the consideration of relationships.
% An example of memorizing new concepts via both is 
In Figure \ref{figure:ml}, intuitively, the utilization of meaningful learning can encourage learners to understand information continuously built on concepts the learners already understand \citep{okebukola1988cognitive}. Following this, we intend to examine models' systematic compositionality by exploring semantic linking that establishes semantic relations between primitives (old concepts) and their variants (new concepts). We propose to spoon-feed semantic knowledge to models for semantic linking in two ways, that is, inductive learning and deductive learning \citep{hammerly1975deduction,shaffer1989comparison,thornbury1999teach}. In this section, we discuss the process of semantic linking and take ``\textit{jump}" from SCAN as an example primitive to illustrate the learning scheme.

% \vspace{-3mm}
\subsection{Semantic links}
% \vspace{-1mm}

We focus on three semantic relationships, namely, \emph{lexical variant}, \emph{co-hyponym}, and \emph{synonym}. Lexical Variant refers to an alternative expression form for the same concept. Co-hyponym is a linguistic term to designate a semantic relation between two group members belonging to the same broader class, where each member is a hyponym and the class is a hypernym \citep{lyons1995linguistic}. Synonym stands for a word, morpheme, or phrase that shares exactly or nearly the same semantics with another one. We provide an example in Figure \ref{figure:ml} and a detailed description in Appendix \ref{appendix:sl}.

% \vspace{-3mm}
\subsection{Inductive learning} \label{sec:il}
% \vspace{-1mm}

Inductive learning is a bottom-up approach from the more specific to the more general. In grammar teaching, inductive learning is a rule-discovery approach starting with the presentation of specific examples from which a general rule can be inferred \citep{thornbury1999teach}. In semantic linking, we propose to introduce variant samples sharing the same context with their primitives during training. The assumption is that models can observe the interchange of primitives and their variants surrounded by the same context in the hope of coming up with a general hypothesis that there is a semantic linking between primitives and their variants \citep{harris1954distributional}. To test the generalization, we design a prompt ``\textit{[concept] twice}'' from a primitive sample ``\textit{jump twice}''. After that, we fill in the concept slot with ``\textit{jump\_0}'' and generate the variant sample ``\textit{jump\_0 twice}''. There is no change from the target side. Finally, by training models on the generated variant sample in combination with prior knowledge (all the other primitive samples), we aim to establish the semantic relationship between ``\textit{jump}'' and ``\textit{jump\_0}'' inductively.
% This process can be treated as a kind of replacement augmentation \citep{wei-zou-2019-eda}.

% \vspace{-3mm}
\subsection{Deductive learning} \label{sec:dl}
% \vspace{-1mm}

Deductive Learning, the opposite of inductive learning, is a top-down approach from the more general to the more specific. As a rule-driven approach, teaching in a deductive manner often begins with presenting a general rule followed by specific examples in practice where the rule is applied \citep{thornbury1999teach}. To align with this definition, we intend to do semantic linking deductively by combining a bilingual dictionary that maps primitives and their variants to the same in the target domain. This additional dictionary, hence, mixes the original training task with word translation \citep{mikolov2013exploiting}. Without any specific context, we hope the model can utilize the general cross-lingual supervised signals as anchor points so as to launch the semantic linking. We want to point out that deductive learning is partially different from \emph{deductive reasoning}. Although there is an overlap, it is not necessary for the former to extract rules from observations like the inference conducted by the latter. In this work, we care more about the learning outcomes, rather than the reasoning process, through empirical evaluations. In practice, given the same example above, we directly make use of primitive ``\textit{jump}'' and its variant ``\textit{jump\_0}'' as the source sequences, as well as the action ``JUMP'' as their identical target sequences. Words and phrases can be treated as text sequences of relatively short length. By exposing both the primitive rule ``\textit{jump}'' $\rightarrow$ ``JUMP'' and the variants rule ``\textit{jump\_0}''$\rightarrow$ ``JUMP'' during training, we aim to build the semantic connections between ``\textit{jump}'' and ``\textit{jump\_0}'' deductively.
% This process is similar to the bilingual dictionary augmentation \citep{arthur-etal-2016-incorporating, nag2020incorporating}.


==> [BlackboxNLP 2022] Revisit Systematic Generalization via Meaningful Learning/4.systematic_generalization.tex <==
\begin{figure*}[t]
    \begin{center}
        \includegraphics[width=\textwidth]{figures/exp0.pdf}
        \vspace{-8mm}
    \end{center}
    \caption{Experiments on SCAN expressing the total training size (left) and the test sequence accuracy (right) when the number of training samples per variant decreases from the complete set (100\%) to a single sample (1).}
\label{figure:exp0}
\vspace{-2mm}
\end{figure*}

% \vspace{-2mm}
\section{Systematic Generalization}
% \vspace{-2mm}

% Although previous ones are more inclined to argue that neural networks fail to match humans in systematic generalization, we focus on the neglected positive side and revisit such algebraic compositionality conditioned on the semantic linking to see whether the conclusion will change. 
The following section specifies the setup and outcome of the experiments. We first employ SCAN as the initial testbed to reproduce the one-shot generalization conditioned on the semantic linking. Then, we examine neural networks' potential to achieve this on SCAN and two real-world tasks of SP, followed by a sensitivity analysis.

% \vspace{-2mm}
\subsection{Datasets}
% \vspace{-1mm}

Some suggest SCAN is not enough to fully verify compositionality \citep{bastings-etal-2018-jump,keysers2020measuring,dankers-etal-2022-paradox}. Thus, we introduce GEO and ADV generated respectively from real SP datasets: Geography and Advising.\footnote{\url{github.com/jkkummerfeld/text2sql-data}} Example inputs and outputs can be found in Table \ref{table:data}.\\
\textbf{SCAN} \citep{lake2017generalization} is a diagnostic dataset proposed to investigate neural networks' compositionality.\footnote{\url{github.com/brendenlake/SCAN}} It includes 20,910 pairs of commands to their instructed actions such as the example in Figure \ref{figure:scan}. We select \{``\textit{jump}", ``\textit{look}", ``\textit{run}", ``\textit{walk}" \} as 4 primitives to be in line with previous works. We focus on lexical variants and create them by adding a suffix that consists of an underline and a unique number. We control the size of the variants set by setting the upper limit of this number. An example variant of ``\textit{jump}” is ``\textit{jump\_0}" and both mean the same action ``JUMP". \\
\textbf{Geography} is a common SP dataset \citep{data-geography-original,data-atis-geography-scholar}, containing 880 examples of queries paired with corresponding expressions. It is later formatted to SQL language with variables in the target sequences \citep{data-sql-advising}. \textbf{GEO} is generated from Geography. We regard 4 of 9 annotated variables as hypernyms and keep them as they are in SQL sequences. The other variables are restored by entities from the source sequence accordingly. As a result, the overall data size is 618 after processing. We can make use of the ``is-a" hypernymy relation for semantic linking. Specifically, we select \{``\textit{new york city}", ``\textit{mississippi rivier}", ``\textit{dc}", ``\textit{dover}" \} as 4 primitives\footnote{We randomly select 4 primitives from GEO and ADV to align with SCAN.} with their variants consisting of entities as co-hyponyms sharing the same variable group with primitives. An example variant of ``\textit{new york city}” is ``\textit{houston city}" and both are in the same variable group ``CITY\_NAME''. \\
\textbf{Advising} includes 4,570 questions on course information paired with SQL queries \citep{data-sql-advising}. \textbf{ADV} is generated from Advising. We treat 4 of 26 annotated variables as hypernyms. Precisely, we select \{ ``\textit{a history of american film}", ``\textit{aaron magid}", ``\textit{aaptis}", ``\textit{100}" \} as 4 primitives with their variants as co-hyponyms sharing the same variables. For instance, ``\textit{advanced at ai techniques}" is a co-hyponym of ``\textit{a history of american film}" sharing the same variable ``TOPIC".

\begin{table*}[t]
  \resizebox{\textwidth}{!}{
  \centering
  \begin{tabular}{llccccccccccccccc}
    \toprule
    & & \multicolumn{5}{c}{SCAN} & \multicolumn{5}{c}{GEO} & \multicolumn{5}{c}{ADV} \\
    \cmidrule(r){3-7}
    \cmidrule(r){8-12}
    \cmidrule(r){13-17}
    \multicolumn{2}{l}{\textbf{Data}} & \multicolumn{3}{c}{Exp. IL} & \multicolumn{2}{c}{Exp. DL} & \multicolumn{3}{c}{Exp. IL} & \multicolumn{2}{c}{Exp. DL} & \multicolumn{3}{c}{Exp. IL} & \multicolumn{2}{c}{Exp. DL} \\
    \cmidrule(r){3-5}
    \cmidrule(r){6-7}
    \cmidrule(r){8-10}
    \cmidrule(r){11-12}
    \cmidrule(r){13-15}
    \cmidrule(r){16-17}
    & & Sta. & Dif. & Cha. & Sta. & Dif. & Sta. & Dif. & Cha. & Sta. & Dif. & Sta. & Dif. & Cha. & Sta. & Dif. \\
    \midrule
    \multicolumn{2}{l}{\textbf{Train Size}} & 20946 & 20942 & 20928 & 20950 & 20946 & 724 & 720 & 711 & 728 & 724 & 6038 & 6034 & 5969 & 6040 & 6036 \\
    \multicolumn{2}{l}{\textbf{Test Size}}  & 308240 & 308240 & 308240 & 308240 & 308240 & 21350 & 21350 & 21350 & 21350 & 21350 & 107614 & 107614 & 107614 & 107614 & 107614 \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-2mm}
  \caption{Dataset statistics for inductive learning (IL) and deductive learning (DL) across Standard (Sta.), Difficult (Dif.), and Challenging (Cha.) in Section \ref{sec:sli}.}
  \label{table:data_il&dl}
\vspace{-2mm}
\end{table*}

% \vspace{-3mm}
\subsection{Models and experimental setup}
% \vspace{-1mm}

% Without specific instruction, settings are shared throughout experiments. \\
\textbf{Models.} After testing many adapted versions, we employ three dominant model candidates, that is, RNN, CNN, and TFM. In terms of RNN, we reproduce bi-directional recurrent networks \citep{schuster1997bidirectional} with long short-term memory units \citep{hochreiter1997long} and an attention mechanism \citep{bahdanau2014neural}. We follow the convolutional seq2seq architecture presented by \citet{gehring2017convolutional} with regard to CNN and the attention-based structure proposed by \citet{NIPS2017_7181} in the case of TFM. More details are in Appendix \ref{appendix:model}. \\
\textbf{Training.} We apply the mini-batch strategy to sample 128 sequence pairs for each training step. We use Adam optimizer \citep{DBLP:journals/corr/KingmaB14} with an $\ell_2$ gradient clipping of $5.0$ \citep{10.5555/3042817.3043083} and a learning rate of 1$e^{-4}$. We freeze the maximum training epoch at 320 for CNN and 640 for RNN and TFM. To prevent uncontrolled interference, we train all models from scratch instead of fine-tuning \citep{devlin-etal-2019-bert}. For the same reason, we break words by whitespace tokenization rather than subword modeling. So, we can guarantee that words are treated separately as distinct tokens with completely different embeddings.\\
\textbf{Evaluation.} Token and sequence accuracy serve as two primary metrics. The former allows partial errors in a sequence, while the latter strictly does not. Every reported number, along with the standard deviation, is the mean of five runs.

% \vspace{-3mm}
\subsection{Experiment: meaningful learning}
% \vspace{-1mm}

Thanks to their incredible algebraic compositionality \citep{chomsky1957syntactic}, humans can effectively capture the underlying semantic connections between new and old concepts and generalize the prior knowledge to novel combinations by meaningful learning \citep{ausubel1963psychology}. To investigate the extent to which models can do the same, we probe the models' compositionality by introducing semantic linking. It is reasonable to illustrate the function of semantic linking through an ablation study, while its missing will lead to an out-of-vocabulary (OOV) issue since there will be no sample to expose variants during training. Replacing variants with other tokens (e.g., “\textit{[unk]}”) goes against our intent to investigate the generalization from primitives to their variants. It also leads to an unfair comparison, where all the variants, for example, go to the same unknown token and cause poor test accuracy. Instead, we gradually remove training samples for each variant until the one-shot learning scenario. We hope to observe the presence of models' meaningful learning by measuring the corresponding performance loss. \\
\textbf{Experimental setup.} Following section \ref{sec:il}, we make use of 40 variants for 4 primitives and produce a total of 329,190 samples, including both primitive and variant samples. We randomly split them into a training set (80\%) and a test set (20\%). The training set is further processed to remove samples having multiple variants to ensure that each variant occurs only once in each sample. Eventually, the training set contains 235,002 samples. Models directly trained on this full dataset serve as baselines. Then, to format a gradual transition from baselines to the meaningful learning, we train the same models on various datasets with a decreasing number of augmented samples for each variant until the one-shot learning setting. Besides, we use the variant rule ``\textit{jump\_0}'' $\rightarrow$ ``JUMP'' as the only training sample for ``\textit{jump\_0}'' in the end as a case of our deductive learning introduced in Section \ref{sec:dl} and consider the rest as our inductive learning. \\
\textbf{Results.} As elaborated in Figure \ref{figure:exp0}, the solid line (SCAN) in green denotes the total training data size against the decreasing number of training samples per variant. The dashed line in other colors denotes the test sequence accuracy against the same horizontal axis. RNN has no significant performance drop when the training size is reduced from 100\% to 1. It still achieves 99.92\% test sequence accuracy when there is only one training sample for each variant. The same happens for CNN and TFM. Despite a slight fluctuation, they keep the results almost consistent regardless of whether the number of training variant samples is all or 1. It is not necessary to augment the training set nearly 14 times from 16,736 to 235,002 to cover all the possible variant compositions. The participation of a single sample is able to launch semantic linking via either inductive learning (a variant sample) or deductive learning (a variant rule), thus enabling models to achieve one-shot generalization. We put two plots in one figure to emphasize such a surprising observation through the strong contrast.

\begin{table*}[t]
  \begin{center}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{llcccccc}
    \toprule
    \multirow{2}{*}{\textbf{Data}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Token Acc.\%}} & \multicolumn{3}{c}{\textbf{Seq. Acc.\%}} \\
    \cmidrule(r){3-5}
    \cmidrule(r){6-8}
    & & \textbf{Standard} & \textbf{Difficult} & \textbf{Challenging} & \textbf{Standard} & \textbf{Difficult} & \textbf{Challenging} \\
    \midrule
     & RNN & $99.99\pm0.03$ & $99.89\pm0.19$ & $99.96\pm0.02$ & $99.95\pm0.08$ & $99.85\pm0.08$ & $99.80\pm0.31$ \\
    SCAN & CNN & $99.96\pm0.08$ & $99.76\pm0.54$ & $98.89\pm2.44$ & $99.85\pm0.34$ & $99.52\pm1.07$ & $97.57\pm5.24$ \\
     & TFM & $98.91\pm0.78$ & $98.90\pm1.10$ & $98.76\pm0.85$ & $97.35\pm1.62$ & $96.86\pm2.64$ & $96.38\pm2.81$ \\
    \midrule
     & RNN & $75.71\pm8.42$ & $75.69\pm6.12$ & $73.46\pm3.05$ & $44.95\pm14.69$ & $43.27\pm13.47$ & $36.77\pm5.60$ \\
    GEO & CNN & $87.99\pm2.67$ & $79.51\pm6.03$ & $77.40\pm2.48$ & $69.46\pm5.78$ & $51.20\pm8.64$ & $48.58\pm3.40$ \\
     & TFM & $75.37\pm7.84$ & $75.11\pm4.88$ & $68.41\pm4.76$ & $45.93\pm12.42$ & $44.59\pm9.76$ & $36.93\pm7.47$ \\
    \midrule
     & RNN & $58.61\pm6.18$ & $59.74\pm5.67$ & $58.11\pm5.82$ & $36.18\pm5.75$ & $35.69\pm6.05$ & $35.45\pm6.69$ \\
    ADV & CNN & $57.83\pm7.55$ & $54.05\pm5.74$ & $53.66\pm2.57$ & $45.08\pm9.32$ & $42.14\pm6.90$ & $41.37\pm4.04$ \\
     & TFM & $53.43\pm2.80$ & $51.51\pm4.50$ & $49.17\pm2.58$ & $42.59\pm3.65$ & $41.28\pm4.35$ & $38.88\pm2.68$ \\
    \bottomrule
  \end{tabular}
  }
  \end{center}
  \vspace{-2mm}
  \caption{Evaluation results over RNN, CNN, and TFM on SCAN, GEO, and ADV across Standard, Difficult, and Challenging in Section \ref{subsec:il}.}
  \label{table:il}
  \vspace{-4mm}
\end{table*}

% \vspace{-2mm}
\subsection{Experiment: semantic linking injection} \label{sec:sli}
% \vspace{-1mm}

% Having observed the presence of meaningful learning, one question that needs to be asked, however, is how it works. 
The following two experiments evaluate models' systematic generalization, particularly for prior knowledge and semantic linking. A sliding scale of difficulty is carefully designed by weakening these two factors according to the assumption that the greater the difficulty, the more compositional skills are required. We further validate our findings on GEO and ADV. We use the same evaluation protocol across different datasets in this section.

Taking the base dataset as prior knowledge, we replace the primitives in source sequences with their variants to generate novel compositions, as introduced in Section \ref{sec:il}. So far, the produced variant samples are not in the training set but in the test set. Hence, variants exist as OOV now. Then, we either incorporate one variant sample to introduce variants in training inductively or one variant rule to do so deductively. In the one-shot learning scenario, we ensure each variant only has a single sample and appears only once during training. For convenience, we keep the same settings for each primitive to have 10 variants in SCAN and a full variant set in GEO (e.g., 39 variants for ``\textit{new york city}"). It is noted in ADV that we randomly sample 5 variants for each primitive so that we cover all the variants with an appropriate test size.

% \vspace{-3mm}
\subsubsection{Inductive learning} \label{subsec:il}
% \vspace{-1mm}

\textbf{Experimental setup.} We increase the difficulty by excluding primitive samples from the training set. It is worth noting that models have to generalize to not only new concepts but also their new compositions with a higher level of difficulty.
\begin{itemize}[leftmargin=*,noitemsep,topsep=0pt]
    \item \textbf{Standard}: Models are trained on prior knowledge and one variant sample per variant.
    \item \textbf{Difficult}: We remove from the prior knowledge primitive samples sharing the same context with their variant samples. For example, we remove ``\textit{jump twice}'' due to ``\textit{jump\_0 twice}'', and thus models have to generalize to ``\textit{jump\_0 twice}'' without seeing ``\textit{jump twice}''.
    \item \textbf{Challenging:} We also exclude from the prior knowledge primitive samples of the same length as their variant samples. For instance, models have to reproduce the same generalization to ``\textit{jump\_0 twice}'' without seeing primitive samples of length 2, including ``\textit{jump twice}'', ``\textit{jump right}'', ``\textit{jump left}", to name a few.\footnote{We remove samples that will not lead to unknown tokens.}
\end{itemize}
\begin{table}[t]
  \begin{center}
  \resizebox{\linewidth}{!}{
  \begin{tabular}{llcccc}
    \toprule
    \multirow{2}{*}{\textbf{Data}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Token Acc.\%}} & \multicolumn{2}{c}{\textbf{Seq. Acc.\%}} \\
    \cmidrule(r){3-4}
    \cmidrule(r){5-6}
    & & \textbf{Standard} & \textbf{Difficult} & \textbf{Standard} & \textbf{Difficult} \\
    \midrule
    & RNN & $99.48\pm0.71$ & $98.70\pm0.92$ & $98.27\pm2.38$ & $95.39\pm2.72$ \\
    SCAN & CNN & $99.99\pm0.01$ & $98.59\pm3.10$ & $99.96\pm0.03$ & $96.66\pm7.27$ \\
    & TFM & $96.90\pm1.78$ & $96.68\pm2.21$ & $91.94\pm4.04$ & $91.26\pm5.80$ \\
    \midrule
    & RNN & $54.44\pm7.15$ & $39.71\pm18.38$ & $13.61\pm7.08$ & $7.76\pm5.34$ \\
    GEO & CNN & $41.86\pm3.38$ & $41.07\pm7.48$ & $4.85\pm4.66$ & $4.04\pm2.18$ \\
    & TFM & $67.02\pm6.91$ & $65.97\pm5.17$ & $36.38\pm10.08$ & $31.57\pm7.42$ \\
    \midrule
    & RNN & $36.50\pm7.66$ & $36.42\pm7.39$ & $12.84\pm4.31$ & $12.66\pm5.19$ \\
    ADV & CNN & $43.51\pm11.31$ & $35.34\pm14.68$ & $32.33\pm12.93$ & $23.58\pm16.04$ \\
    & TFM & $56.82\pm3.79$ & $53.33\pm3.85$ & $47.43\pm3.71$ & $43.24\pm5.14$ \\
    \bottomrule
  \end{tabular}
  }
  \end{center}
  \vspace{-2mm}
  \caption{Evaluation results over RNN, CNN, and TFM on SCAN, GEO, and ADV across Standard and Difficult in Section \ref{subsec:dl}.}
  \label{table:dl}
\vspace{-4mm}
\end{table}
\textbf{SCAN.} What stands out in Table \ref{table:il} is an excellent one-shot generalization for all three networks. The participation of variant samples induces a near-perfect generalization. Even the worst results obtained by TFM in Challenging are around $98.76\%$ and $96.38\%$ in terms of token and sequence accuracy. The outcomes confirm that networks can inductively learn semantic relations from the context after semantic linking. The disappearance of training samples in Difficult and Challenging causes a performance drop. This is well in line with the widely accepted belief in meaningful learning theory that prior knowledge matters to generalization. \\
\textbf{GEO \& ADV.} The more apparent changes in metrics again verify that prior knowledge is essential. Either excluding primitive samples containing the same context or those of the same sequence length can produce a steep fall in the generalization. On GEO, CNN can lose an absolute sequence accuracy of $18.26\%$ from Standard to Difficult, and that for TFM drops $7.66\%$. This upholds our argument that generalization via meaningful learning is inseparable from sufficient prior knowledge. The overall decline in performance can be attributed to the switch from toy sets to actual datasets since both GEO and ADV own a much more complex encoding and decoding space than SCAN. Therefore, we conclude that both prior knowledge and semantic linking exert powerful effects upon the potential of models to generalize systematically.

% \vspace{-2mm}
\subsubsection{Deductive learning} \label{subsec:dl}
% \vspace{-1mm}

\textbf{Experimental setup.} We increase the difficulty of compositional learning by excluding primitive rules from the training set as follows:
\begin{itemize}[leftmargin=*,noitemsep,topsep=0pt]
    \item \textbf{Standard}: Models are trained on the prior knowledge, primitive rules, and variant rules.
    \item \textbf{Difficult}: We remove primitive rules from the training set. Consequently, semantic links are weakened and depend on variant rules only.
\end{itemize}
\textbf{SCAN.} By incorporating deductive semantic linking, all three networks attain satisfying compositional generalization as shown in Table \ref{table:dl}. CNN achieves the highest $99.96\%$ in Standard, while TFM takes the lowest $91.26\%$ in Difficult with regard to sequence accuracy. We can see a consistent decline in accuracy when we undermine the semantic linking by removing primitive rules from the training set. The most significant sequence accuracy drop of $3.3\%$ comes from CNN when the difficulty upgrades. However, in Difficult, even the lowest one is impressive as there is only one variant rule to introduce each variant during training. \\
\textbf{GEO \& ADV.} There is a persistent performance loss because of the absence of primitive rules from the training set across models. Concretely in GEO, the grade of CNN declines from $32.33\%$ in Standard to $23.58\%$ in Difficult in terms of sequence accuracy. The causal role of semantic linking is also demonstrated by varying the difficulty. The difference between Standard and Difficult indicated that either concept rules and just variant rules can connect primitives with their variants semantically, though the former is better than the latter. Moreover, models appear to realize systematic generalization better in an inductive way. By comparing Table \ref{table:il} with Table \ref{table:dl}, we find that current black-box neural nets are more capable of exploring patterns from specific samples with context information rather than understanding knowledge from general rules in our experiments. This sheds light on why current machine learning is still highly data-driven and can hardly break through the bottleneck to conduct advanced logic reasoning as human beings.

\begin{figure}[t]
    \begin{center}
        \includegraphics[width=\linewidth]{figures/sa.pdf}
        \vspace{-8mm}
    \end{center}
\caption{Experiments over RNN on SCAN with varying \#primitives (a) and \#variants (b).}
\label{figure:sa}
\vspace{-2mm}
\end{figure}

% \vspace{-2mm}
\subsection{Sensitivity analysis} \label{sec:sa}
% \vspace{-1mm}

\begin{table*}[t]
  \resizebox{\textwidth}{!}{
  \centering
  \begin{tabular}{lcccccccc}
    \toprule
     & \multicolumn{4}{c}{\textbf{IWSLT'14}} & \multicolumn{4}{c}{\textbf{IWSLT'15}} \\
    \cmidrule(r){2-5}
    \cmidrule(r){6-9}
    \textbf{Model} & \multicolumn{2}{c}{\textbf{En-De}} & \multicolumn{2}{c}{\textbf{De-En}} & \multicolumn{2}{c}{\textbf{En-Fr}} & \multicolumn{2}{c}{\textbf{Fr-En}} \\
    \cmidrule(r){2-3}
    \cmidrule(r){4-5}
    \cmidrule(r){6-7}
    \cmidrule(r){8-9}
     & \textbf{BLEU} & \textbf{SacreBLEU} & \textbf{BLEU} & \textbf{SacreBLEU} & \textbf{BLEU} & \textbf{SacreBLEU}  & \textbf{BLEU} & \textbf{SacreBLEU} \\
    \midrule
    \multicolumn{9}{l}{\textbf{Baselines}} \\
    LSTM \citep{luong-etal-2015-effective} & 24.98 & 24.88 & 30.18 & 32.62 & 38.06 & 42.93 & 37.34 & 39.36 \\
    Transformer \citep{NIPS2017_7181} & 28.95 & 28.85 & 35.24 & 37.60 & 41.82 & 46.41 & 40.45 & 42.61 \\
    Dynamic Conv. \citep{wu2018pay} & 27.39 & 27.28 & 33.33 & 35.54 & 40.41 & 45.32 & 39.61 & 41.42 \\
    \midrule
    \multicolumn{9}{l}{\textbf{\texttt{\Large+}Vocabulary Augmentation}} \\
    LSTM \citep{luong-etal-2015-effective} & 25.35$\uparrow_{0.37}$ & 25.38$\uparrow_{0.50}$ & 30.99$\uparrow_{0.81}$ & 33.63$\uparrow_{1.01}$ & 38.32$\uparrow_{0.26}$ & 43.30$\uparrow_{0.37}$ & 37.77$\uparrow_{0.43}$ & 39.83$\uparrow_{0.47}$ \\
    Transformer \citep{NIPS2017_7181} & 29.40$\uparrow_{0.45}$ & 29.29$\uparrow_{0.44}$ & 35.72$\uparrow_{0.48}$ & 38.07$\uparrow_{0.47}$ & 42.19$\uparrow_{0.37}$ & 46.68$\uparrow_{0.27}$ & 41.04$\uparrow_{0.59}$ & 43.15$\uparrow_{0.54}$ \\
    Dynamic Conv. \citep{wu2018pay} & 27.60$\uparrow_{0.21}$ & 27.50$\uparrow_{0.22}$ & 33.62$\uparrow_{0.29}$ & 36.00$\uparrow_{0.46}$ & 40.87$\uparrow_{0.46}$ & 45.95$\uparrow_{0.63}$ & 39.95$\uparrow_{0.34}$ & 41.86$\uparrow_{0.44}$ \\
    \bottomrule
  \end{tabular}}
  \vspace{-2mm}
  \caption{Evaluation results over LSTM, Transformer, and Dynamic Conv. on IWSLT'14 En-De (English-German) and De-En, IWSLT'15 En-Fr (English-French) and Fr-En translations.}
  \label{table:mt}
\vspace{-4mm}
\end{table*}

Regarding deductive learning, we conduct sensitivity analysis with a varying number of primitives (\#primitives) from \{1,2,3,4\} and that of variants per primitive (\#variants) from \{1,5,10,15,20\} over RNN on SCAN. The experimental setup is borrowed from Standard in Section \ref{subsec:dl}. \\
\textbf{Impact of \#primitives.} In Figure \ref{figure:sa} (a), the generalization performance improves w.r.t. accuracy boosting and variance reduction when \#primitives grows simultaneously. This is counter-intuitive as we thought primitive rules should work independently. A potential reason is semantic linking built by various \emph{independent} primitive rules can profit each other to trigger a more robust and stable generalization. For example, ``\textit{jump}'' $\rightarrow$ ``JUMP'' and ``\textit{look}'' $\rightarrow$ ``LOOK'' may separate them from the context such as ``\textit{\textbf{jump} right}'' and ``\textit{\textbf{look} right}''. So, ``\textit{[concept] right}'' functions as a compositional rule shared among primitive samples and finally encourages models to generalize more effectively. \\
\textbf{Impact of \#variants.} As presented in Figure \ref{figure:sa} (b), RNN generalizes consistently well when \#variants goes up. Therefore, we report that the generalization among variants of the same primitive has a certain degree of independence within a reasonable range (e.g., \#variants $\leq 20$).

==> [BlackboxNLP 2022] Revisit Systematic Generalization via Meaningful Learning/5.discussion.tex <==
% \vspace{-2mm}
\section{From SCAN to Real Data}
% \vspace{-2mm}

Thus far, we have argued the feasibility of systematic generalization activated by semantic linking. We move on to discuss how it already benefits machines in solving real problems. Many recent papers propose to improve systematic generalization by techniques such as data augmentation \citep{andreas-2020-good,rek2021learning} and meta-learning \citep{NEURIPS2019_f4d0e2e7,conklin-etal-2021-meta}. The success is reasonable given our findings. Replacing fragments in real training samples with others that share similar contexts is supported by our inductive learning. We have demonstrated that similar context information can help establish the semantic links between new concepts and old ones, thus enabling models to generalize compositionally. By considering concepts as pointers in the memory, meta-learning equips models with memory loading to make connections between new and old concepts as semantic linking. The utility of similar unsupervised techniques \citep{xie2019unsupervised} in both compositional generalization and real tasks can be attributed to inductive learning as well. Besides, our sensitivity analysis in Section \ref{sec:sa} shows that adding seemingly independent primitive samples or rules can also improve the generalization, which has been further validated recently \citep{auersperger-pecina-2021-solving,patel-etal-2022-revisiting}.

In addition to inductive-based methods, some works \citep{mikolov2013exploiting,arthur-etal-2016-incorporating, nag2020incorporating}, incorporating bilingual dictionaries in low-resource MT, can fall in the field of deductive-based ones. As a proof-of-concept, we reproduce the word-to-word augmentation, or called deductive learning in this work, by training models on not only the base training set but also concept rules. Intuitively, we wonder to which extent deductive semantic linking can promote models' performance in MT (IWSLT'14 and IWSLT'15) and SP (Geography and Advising). We report the evaluation results in Table \ref{table:mt} and Table \ref{table:sp}. Details of models and data can be found in Appendix \ref{appendix:model} and Appendix \ref{appendix:data}.

\begin{table*}[t]
  \resizebox{\textwidth}{!}{
  \centering
  \begin{tabular}{lcccccccc}
    \toprule
     & \multicolumn{4}{c}{\textbf{Geography}} & \multicolumn{4}{c}{\textbf{Advising}} \\
    \cmidrule(r){2-5}
    \cmidrule(r){6-9}
    \textbf{Model} & \multicolumn{2}{c}{\textbf{Train}} & \multicolumn{2}{c}{\textbf{Test}} & \multicolumn{2}{c}{\textbf{Train}} & \multicolumn{2}{c}{\textbf{Test}} \\
    \cmidrule(r){2-3}
    \cmidrule(r){4-5}
    \cmidrule(r){6-7}
    \cmidrule(r){8-9}
     & \textbf{Token Acc.\%} & \textbf{Seq. Acc.\%} & \textbf{Token Acc.\%} & \textbf{Seq. Acc.\%} & \textbf{Token Acc.\%} & \textbf{Seq. Acc.\%} & \textbf{Token Acc.\%} & \textbf{Seq. Acc.\%} \\
    \midrule
    \multicolumn{8}{l}{\textbf{Baselines}} \\
    RNN & 89.05 & 17.39 & 69.81 & 9.68 & 92.22 & 3.64 & 60.41 & 6.11 \\
    CNN & 98.45 & 70.74 & 78.44 & 55.91 & 99.74 & 81.62 & 81.74 & 51.13 \\
    TFM & 99.45 & 84.95 & 80.24 & 49.82 & 99.68 & 76.90 & 78.51 & 29.67 \\
    \midrule
    \multicolumn{8}{l}{\textbf{\texttt{\Large+}Entity Augmentation}} \\
    RNN & 87.47 & 29.96 & 72.39$\uparrow_{2.58}$ & 15.05$\uparrow_{5.37}$ & 88.82 & 30.97 & 71.17$\uparrow_{10.76}$ & 16.06$\uparrow_{9.95}$ \\
    CNN & 97.54 & 76.03 & 80.32$\uparrow_{1.88}$ & 60.93$\uparrow_{5.02}$ & 99.65 & 87.01 & 84.50$\uparrow_{2.76}$ & 56.02$\uparrow_{4.89}$ \\
    TFM & 99.30 & 85.73 & 81.09$\uparrow_{0.85}$ & 54.84$\uparrow_{5.02}$ & 99.57 & 86.94 & 84.26$\uparrow_{5.75}$ & 35.08$\uparrow_{5.41}$ \\
    \bottomrule
  \end{tabular}}
  \vspace{-2mm}
  \caption{Evaluation results over RNN, CNN, and TFM on Geography and Advising.}
  \label{table:sp}
\vspace{-4mm}
\end{table*}

\subsection{Machine translation}
\textbf{Setup.}
We evaluate our approach on IWSLT'14 \cite{cettolo2014report} English-German (En-De) and German-English (De-En), IWSLT'15 \cite{Cettolo2015TheI2} English-French (En-Fr) and French-English (Fr-En) translation tasks. We follow the standard evaluation protocol \cite{ott2019fairseq} that keeps the original training set and validation set but combines multiple previous test sets for final evaluation. The test set of IWSLT'14 consists of IWSLT14.TED.dev\{2010, 2012\} and IWSLT14.TED.tst\{2010, 2011, 2012\}. That of IWSLT'15 includes IWSLT15.TED.tst\{2014, 2015\} \cite{ott2019fairseq}. We apply BPE with 10K tokens for all tasks and report both BLEU \cite{papineni2002bleu} and SacreBLEU \cite{post-2018-call} scores for three baselines: LSTM \cite{luong-etal-2015-effective}, Transformer \cite{NIPS2017_7181}, and Dynamic Conv. \cite{wu2018pay} in comparsion with same structures augmented by our method.
\\
\textbf{Vocabulary augmentation.}
We introduce concept rules as \emph{vocabulary augmentation} in MT. The semantic links between primitives and their variants can be built upon the synonymous relations between tokens such as ``\textit{heavily populated}" and ``\textit{populous}". From this, the source words paired with translated ones can be regarded as concept rules. It is noted that such relationships are reversible as shown in Figure \ref{figure:ml}, so a primitive can be a variant of the other primitive as well. In practice, we collect a dictionary of tokens in the source language and feed them to the Google Translation\footnote{\url{cloud.google.com/translate}} so as to obtain a token map from the source language to the target one. The same operation can be repeated from the target language to the source one. Two dictionaries are combined into one with duplicates removed. Consequently, we get 144,874 token-level samples as a training supplementary for IWSLT'14 En-De and De-En, and 110,099 for IWSLT'15 En-Fr and Fr-En, which leads to a total of 305,113 training samples for IWSLT'14 En-De and De-En and 315,671 for IWSLT'15 En-Fr and Fr-En after such vocabulary augmentation.
\\
\textbf{Results.}
From Table \ref{table:mt}, we observe a consistent improvement in both BLEU and SacreBLEU over all baselines after vocabulary augmentation, particularly up to 1 in SacreBlEU. The additional synonym pairs not only construct the semantic linking between tokens in two languages explicitly, but also create a complicated semantic linking network implicitly because of synonyms within the single language and the transitivity nature of synonym relation. Our experiments prove that semantic linking, which allows models to generalize systematically, can be beneficial for improving MT performance.

\subsection{Semantic parsing}
\textbf{Setup.}
We evaluate our method on two SP benchmarks, Geography, and Advising. We train the same models (i.e., RNN, CNN, and TFM) as we analyzed before without further hyperparameter tuning. There are some changes for CNN, where the learning rate is 5$e^{-4}$ in Geography, and the maximum sequence length for the decoder position embedding is 312 in Advising. We split $10\%$ training samples as the validation set to find the converged epoch and then add it back to the training set for the final report.
\\
\textbf{Entity augmentation.}
We introduce concept rules as \emph{entity augmentation} in SP. The semantic links are established among co-hyponyms. We consider a variable as a hypernym for its values. By that, entities belonging to the same variable are co-hyponyms. Thus, we can regard entity values as primitives and the translations from primitives (e.g., ``\textit{new york city}'') to their variables (e.g., ``CITY\_NAME'') as primitive rules. To be specific, We construct entity dictionaries by collecting entities such as ``\textit{new york city}''. They are translated to themselves since they do not change from the source natural language to the target SQL. For a fair comparison, a token from this extra dataset will be marked as a unique unknown mark, ``\textit{[unk]}", if it does not exist in the original base training set. After that, we have a map of 103 entity translations for  Geography and 1846 for Advising, resulting in a training size change from 701 to 804 for Geography and from 3814 to 5660 for Advising.
\\
\textbf{Results.}
As elaborated in Table \ref{table:sp}, all three networks can achieve better performance in terms of both accuracy and variance. A $10.76\%$ token accuracy and $9.95\%$ sequence accuracy boosting are observed from RNN on Advising after such entity augmentation. The results suggest that models can learn semantic linking or be more familiar with similar contexts from those primitive rules in a deductive way to enhance model systematic generalization and finally lead to better outcomes. 

==> [BlackboxNLP 2022] Revisit Systematic Generalization via Meaningful Learning/6.conclusion.tex <==
% \vspace{-2mm}
\section{Conclusion}
% \vspace{-2mm}

We revisit systematic generalization from a meaningful learning perspective. According to the theory, we conduct semantic linking to expose semantic relations between new and old concepts via either inductive learning or deductive learning. Experimental results on SCAN, GEO, and ADV support that seq2seq neural networks, as a class of modern machine learning methods, can behave systematically after semantic linking. Testing with various difficulties indicates that both semantic linking and prior knowledge are two essential factors in such generalization, in agreement with what humans do in meaningful learning. Finally, we group recent methods in either the inductive-based or deductive-based category, followed by a proof-of-concept, to highlight the already-existing advantages of meaningful learning in applications such as machine translation and semantic parsing.

We want to underline that, to the best of our knowledge, this work is the first one exploring the optimistic results observed by \citet{lake2017generalization}. Our positive findings oppose the recent prevailing view that neural networks appear inherently ineffective in such cognitive capacity, thus confirming the mixed picture. By rationalizing recent findings from a meaningful learning perspective, we hope to encourage followers to interpret the exceptional generalization ability through the connection between neural nets and human cognition.



==> [BlackboxNLP 2022] Revisit Systematic Generalization via Meaningful Learning/7.others.tex <==
\section*{Limitations}
We establish semantic relationships between primitives and their variants by either inductive or deductive learning. The incorporation of both learning skills is worth exploring further. We primarily utilize data augmentation techniques to expose the semantic information to models. Apart from that, there should be many other methods to achieve the same goal. Which method is most appropriate to realize semantic linking remains an open topic. Meanwhile, the application of meaningful learning to promote systematic generalization in practice (e.g., MT and SP) could have been expanded.

\section*{Acknowledgements}
We gratefully appreciate Yewen Pu, Guan (Royal) Wang, Yichen Gong, Rong Zhang, and Hui Xue for sharing their pearls of wisdom. We also would like to express our special thanks of graitude to Yingying Huo for the support, as well as BlackboxNLP anonymous reviewers for their constructive feedback. This work was supported by Shining Lab, Learnable, Inc., and Alibaba Group.
